On the elastic anatomy of heterogeneous fractures in rock

This study examines the feasibility of the full-field ultrasonic characterization of fractures in rock. To this end, a slab-like specimen of granite is subjected to in-plane, O(10$^4$Hz) excitation while monitoring the induced 2D wavefield by a Scanning Laser Doppler Vibrometer (SLDV) with sub-centimeter spatial resolution. Upon suitable filtering and interpolation, the observed wavefield is verified to conform with the plane-stress approximation and used to: (i) compute the maps of elastic modulus in the specimen (before and after fracturing) via a rudimentary application of the principle of elastography; (ii) reconstruct the fracture geometry; (iii) expose the fracture's primal (traction-displacement jump) contact behavior, and (iv) identify its profiles of shear and normal specific stiffness. Through the use of full-field ultrasonic data, the approach provides an unobscured, high-resolution insight into the fracture's contact behavior, foreshadowing in-depth laboratory exploration of interdependencies between the fracture geometry, aperture, interphase properties, and its seismic characteristics.

==> macros.tex <==
%%%\
%%%   Macros (mostly for mathematical formulas)
%%%
\newlength{\kaka}
\newcommand{\dd}[1]{\protect\settowidth{\kaka}{\mbox{$#1$}}\makebox[\kaka]{$\buildrel{\scriptscriptstyle}\over{#1}$}}
\newcommand{\ahref}[2]{}
\newcommand{\der}[2]{\frac{d#1}{d#2}}
\newcommand{\Tsup}{^{\text{\tiny T}}}
\newcommand{\Rsub}{_{\text{\tiny R}}}
\newcommand{\Isub}{_{\text{\tiny I}}}
\newcommand{\Isup}{^{\text{\tiny I}}}
\newcommand{\Esup}{^{\text{\tiny E}}}
\newcommand{\Zsup}{^{\text{\tiny o}}}
\newcommand{\Zsub}{_{\text{\tiny o}}}
\newcommand{\zsub}{_{\!\text{\tiny o}}}
\newcommand{\hard}{_{\text{hard}}}
\newcommand{\soft}{_{\text{soft}}}
\newcommand{\obs}{^{\text{obs}}}
\newcommand{\opt}{_{\text{\tiny{opt}}}}
\newcommand{\true}{^{\text{\tiny true}}}
\newcommand{\eps}{\epsilon}
\newcommand{\px} {\accentset{\star}{p}}
\newcommand{\fx} {\accentset{\star}{f}}
\newcommand{\gx} {\accentset{\star}{g}}

\newcommand{\Sf}{S^{\text{\tiny f}}}
\newcommand{\Sb}{S^{\text{\tiny b}}}
\newcommand{\Lf}{L^{\text{\tiny f}}}


\newcommand{\one}{_{\text{\tiny I}}}
\newcommand{\two}{_{\text{\tiny I\nxs I}}}

\newcommand{\jed}{{\text{I}}}
\newcommand{\dva}{{\text{I\nxs I}}}

\newcommand\mya[1]{\alpha^{#1}}
\newcommand\eqa[1]{\ensuremath{\mathop{\overset{\mya{#1}}{=}}}}% Unscaled version
\newcommand\eqvara[1]{\mathop{\overset{\mya{#1}}{\resizebox{\widthof{\eqa{#1}}}{\heightof{=}}{=}}}}

\newcommand\myk[1]{k^{#1}}
\newcommand\eqk[1]{\ensuremath{\mathop{\overset{\myk{#1}}{=}}}}% Unscaled version
\newcommand\eqvark[1]{\mathop{\overset{\myk{#1}}{\resizebox{\widthof{\eqk{#1}}}{\heightof{=}}{=}}}}

\newcommand\mye[1]{\epsilon^{#1}}
\newcommand\eqe[1]{\ensuremath{\mathop{\overset{\mye{#1}}{=}}}}% Unscaled version
\newcommand\eqvare[1]{\mathop{\overset{\mye{#1}}{\resizebox{\widthof{\eqe{#1}}}{\heightof{=}}{=}}}}

\newcommand\eqqo{\ensuremath{\mathop{\overset{1}{=}}}}% Unscaled version

\newcommand\eqvar{\stackrel{\alpha}{=}}
\newcommand\eqvarm[1]{\stackrel{\alpha^{#1}}{=}}

\newcommand{\lcba}{\left\{\rule{0cm}{0.50cm}\hspace{-0.1cm}\right.}
\newcommand{\rcba}{\left.\hspace{-0.1cm}\rule{0cm}{0.50cm}\right\}} 

\newcommand{\lsba}{\left(\rule{0cm}{0.50cm}\hspace{-0.1cm}\right.}
\newcommand{\rsba}{\left.\hspace{-0.1cm}\rule{0cm}{0.50cm}\right)}

\newcommand{\lcbc}{\left\{\rule{0cm}{0.35cm}\hspace{-0.1cm}\right.}
\newcommand{\rcbc}{\left.\hspace{-0.1cm}\rule{0cm}{0.35cm}\right\}}

\newcommand{\lsqba}{\left[\rule{0cm}{0.50cm}\hspace{-0.1cm}\right.}
\newcommand{\rsqba}{\left.\hspace{-0.1cm}\rule{0cm}{0.50cm}\right]}

\newcommand{\lsqbc}{\left[\rule{0cm}{0.40cm}\hspace{-0.1cm}\right.}
\newcommand{\rsqbc}{\left.\hspace{-0.1cm}\rule{0cm}{0.40cm}\right]}

\newcommand{\lsbc}{\left(\rule{0cm}{0.35cm}\hspace{-0.1cm}\right.}
\newcommand{\rsbc}{\left.\hspace{-0.1cm}\rule{0cm}{0.35cm}\right)}

\newcommand{\lsbb}{\left(\rule{0cm}{0.40cm}\hspace{-0.1cm}\right.}
\newcommand{\rsbb}{\left.\hspace{-0.1cm}\rule{0cm}{0.40cm}\right)}

\newcommand{\lqbb}{\left[\rule{0cm}{0.40cm}\hspace{-0.1cm}\right.}
\newcommand{\rqbb}{\left.\hspace{-0.1cm}\rule{0cm}{0.40cm}\right]}

\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\lb}{\label}
\newcommand{\nn}{\nonumber}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}
\newcommand{\bxr}{\begin{array}}
\newcommand{\exr}{\end{array}}

\newcommand\exs{\hspace*{0.4mm}}
\newcommand\xxs{\hspace*{0.2mm}}
\newcommand\nes{\hspace*{-0.4mm}}
\newcommand\nxs{\hspace*{-0.2mm}}
\newcommand\nms{\hspace*{-0.3mm}}

\newcommand{\Ncal}{\mathcal{N}}
\newcommand{\Ctm}{\mathcal{C}\two}

\def\asym{\mathop{\rm Asym}}
\newcommand{\abs}[1]{\left| #1 \right|}  
\newcommand{\norms}[1]{\parallel\! #1 \!\parallel} 
\newcommand{\inv}[1]{\frac{1}{#1}}
\newcommand{\nnum}{\notag \\}
\newcommand{\suite }{\nnum & \mbox{}\hspace{15pt}}
\newcommand{\bfna}{\nabla}
\newcommand{\demi} {\inv{2}}
\newcommand{\bfG} {\boldsymbol{G}}
\newcommand{\bA} {\boldsymbol{A}}
\newcommand{\bU} {\boldsymbol{U}}
\newcommand{\bSig} {\boldsymbol{\Sigma}}
\newcommand{\bW} {\boldsymbol{W}}
\newcommand{\bC} {\boldsymbol{C}}
\newcommand{\bK} {\boldsymbol{K}}
\newcommand{\bV} {\boldsymbol{V}}
\newcommand{\bJ} {\boldsymbol{J}}
\newcommand{\bM} {\boldsymbol{M}}
\newcommand{\bQ} {\boldsymbol{Q}}
\newcommand{\bH} {\boldsymbol{H}}
\newcommand{\bn} {\boldsymbol{n}}
\newcommand{\ba} {\boldsymbol{a}}
\newcommand{\bb} {\boldsymbol{b}}
\newcommand{\bfn} {\boldsymbol{n}}
\newcommand{\bfP} {\boldsymbol{P}}
\newcommand{\bq} {{\boldsymbol{q}}}
\newcommand{\ff}{^{\text{\tiny f}}}
\newcommand{\bfPt} {\dd{\bfP}}
\newcommand{\bfp} {\boldsymbol{p}}
\newcommand{\bfe} {\boldsymbol{e}}
\newcommand{\bfw} {w}
\newcommand{\bx} {\boldsymbol{x}}
\newcommand{\by} {\boldsymbol{y}}
\newcommand{\be} {\boldsymbol{e}}
\newcommand{\bz} {\boldsymbol{z}}
\newcommand{\bg} {{\boldsymbol{g}}}
\newcommand{\bgt} {\tilde{\bg}}
\newcommand{\ii} {\textrm{i}}
\newcommand{\oG} {\overline{G}}
\newcommand{\bxb} {\bar{\boldsymbol{x}}}
\newcommand{\bm} {\boldsymbol{m}}
\newcommand{\bfx} {\boldsymbol{x}}
\newcommand{\bfX} {\boldsymbol{X}}
\newcommand{\bfXt} {\dd{\bfX}}
\newcommand{\bft} {\boldsymbol{t}}
\newcommand{\bfT} {\boldsymbol{T}}
\newcommand{\bfTt} {\tilde{\bfT}}
\newcommand{\vr} {\tilde{u}{}^{\eps}}
\newcommand{\bftr} {\tilde{\bft}{}^{\eps}}
%\newcommand{\bu} {p}
\newcommand{\bp} {\boldsymbol{p}}
\newcommand{\bfu} {u}
\newcommand{\bfv} {\boldsymbol{v}}
\newcommand{\bd} {\boldsymbol{d}}
\newcommand{\bI} {\boldsymbol{I}}
\newcommand{\bfA} {\boldsymbol{A}}
\newcommand{\bfU} {\boldsymbol{U}}
\newcommand{\bfV} {\boldsymbol{V}}
\newcommand{\bfUt} {\dd{\bfU}}
\newcommand{\bfF} {\boldsymbol{F}}
\newcommand{\AS}{\mbox{\boldmath $\Acal$}}
\newcommand{\US}{\mbox{\boldmath $\Ucal$}}
\newcommand{\bxo} {\bfx\Zsup}
\newcommand{\ro} {r\zsub}
\newcommand{\bzzo} {\boldsymbol{z}\Zsup}
\newcommand{\bxx} {\bzet^{x}}
\newcommand{\rZ} {r\Zsup}
\newcommand{\sym}{^{\text{sym}}}
\newcommand{\bfuo} {\bfu\obs}
\newcommand{\tpe}{\tilde{p}^{\eps}}
\newcommand{\tp}{\tilde{p}}
\newcommand{\tq}{\tilde{q}}
\newcommand{\pe}{p^{\eps}}
\newcommand{\pff}{\boldsymbol{u}^{\textit{i}}}
\newcommand{\qf}{q^{\mbox{\tiny{F}}}}
\newcommand{\po} {u\obs}
\newcommand{\ptr} {p^{\text{true}}}
\newcommand{\bfvo} {\bfv\obs}
\newcommand{\bfsigt} {\dd{\bfsig}}
\newcommand{\bfSigt} {\dd{\bfSig}}
\newcommand{\bksi} {\boldsymbol{\xi}}
\newcommand{\bzet} {\boldsymbol{\zeta}}
\newcommand{\betta} {\boldsymbol{\eta}}
\newcommand{\bksib}{\bar{\boldsymbol{\xi}}}
\newcommand{\xib}{\bar{\xi}}
\newcommand{\kb}{\bar{k}}
\newcommand{\bfxi}{\boldsymbol{\xi}}
\newcommand{\bfxb}{\bar{\bfx}} 
\newcommand{\bfxib}{\bar{\bfxi}}
\newcommand{\xb} {\bar{x}}
\newcommand{\bfW} {\boldsymbol{W}}
\newcommand{\bfeps}{\boldsymbol{\varepsilon}}
\newcommand{\bfpsi}{\boldsymbol{\psi}}
\newcommand{\bfphi}{\boldsymbol{\phi}}
\newcommand{\bfsig}{\boldsymbol{\sigma}}
\newcommand{\bfSig}{\boldsymbol{\Sigma}}
\newcommand{\Acal}{\mathcal{A}}
\newcommand{\Bcal}{\mathrsfs{B}}
\newcommand{\Jcal}{J}
\newcommand{\JCal}{\Jcal_{\!f}}
\newcommand{\Gcal}{\mathcal{G}}
\newcommand{\Lcal}{\mathcal{L}}
\newcommand{\Ocal}{\mathfrak{O}}
\newcommand{\Tcal}{{\sf T}}
\newcommand{\TCal}{\Tcal_{\!f}}
\newcommand{\TCalo}{\Tcal_{\!f\!\text{,\tiny opt}}}
\newcommand{\TCalom}{\Tcal_{\!f\!\text{,\tiny opt}}^{\text{\tiny min}}}
\newcommand{\Ucal}{\mathcal{U}}

\newcommand{\bcc} {\boldsymbol{c}}
\newcommand{\bdo}{\bd^{\hspace*{0.2mm} \text{\tiny o}}}
\newcommand{\sop}{{\text{\tiny o}}}  
\newcommand{\hbs} {\hat{\boldsymbol{s}}}
\newcommand{\hbt} {\hat{\boldsymbol{t}}}
\newcommand{\RR}{\mathbb{R}}

\newcommand{\ropm}{r\one^{\mbox{\tiny{$\pm$}}}}
\newcommand{\rtp}{r\two^{\mbox{\tiny{$+$}}}}
\newcommand{\rtm}{r\two^{\mbox{\tiny{$-$}}}}

\newcommand{\Gc}{\mathcal{G}}
\newcommand{\Hc}{\mathcal{H}}

\newcommand{\Scal}{\mathrsfs{S}}
\newcommand{\dip} {\! :\!}
\newcommand{\sip} {\!\cdot\!}
\newcommand{\derp}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\oo} {\omega}
\newcommand{\OOr}{\OO^{-}_{\eps}}
\newcommand{\OO}{\Omega}
\newcommand{\OOm}{\Omega^{-}}
\newcommand{\OOc}{\Omega_{c}}
\newcommand{\So}{S\obs}
\newcommand{\Sos}{\Gamma\obs_{\!\Sigma}}
\newcommand{\Soo}{\Gamma\obs_{\!\Omega}}
\newcommand{\OOt}{\Omega\true}
\newcommand{\G}{\Gamma}
\newcommand{\Gt}{\G\true}
\newcommand{\bfuG}{\bfu^{c}}
\newcommand{\bftG}{\bft^{c}}
\newcommand{\uG}{u^{c}}
\newcommand{\tG}{t^{c}}
\newcommand{\bfur}{p^{\eps}}
\newcommand{\bfsigr}{\bfsig^{\eps}}
\newcommand{\bfvr}{\tilde{\bfu}{}^{\eps}}
\newcommand{\bfvrS}{\bfvr_{\SN}}
\newcommand{\bftrS}{\bftr_{\SD}}
\newcommand{\bfvrG}{\bfvr_{\Gr}}
\newcommand{\bfut} {\dd{\bfu}}
\newcommand{\bfvt} {\tilde{\bfv}}
\newcommand{\bfutr} {\bfut{}^{\eps}}
\newcommand{\bfvtr} {\bfvt{}^{\eps}}
\newcommand{\bfpt} {\dd{\bfp}}
\newcommand{\bftt} {\dd{\bft}}
\newcommand{\Sigt} {\dd{\Sigma}}
\newcommand{\sigt} {\dd{\sigma}}
\newcommand{\tilU} {\dd{U}}
\newcommand{\tilu} {\dd{u}}
\newcommand{\tilp} {\dd{p}}

\newcommand{\dGG}{\;\text{d}\G}
\newcommand{\dthxi}{\;\text{d}\vartheta_{\xib}}
\newcommand{\dVxi}{\;\text{d}V_{\xib}}
\newcommand{\dOO}{\;\text{d}\OO}
\newcommand{\iS}{\int_{\Scal}}
\newcommand{\Br} {B_{\eps}}
\newcommand{\Sr} {S_{\eps}}
\newcommand{\Gr} {\G_{\eps}}
\newcommand{\Brb} {\overline{B_{\eps}}}
\newcommand{\iBr} {\int_{\Br}}
\newcommand{\iGr} {\int_{\Gr}}

\newcommand{\sd}{\Sigma_{\text{\tiny D}}}
\newcommand{\sn}{\Sigma_{\text{\tiny N}}}

\newcommand{\Bi}{\mathcal{B}_1}
\newcommand{\Bo}{\mathcal{B}_2}
\newcommand{\Bb}{\mathcal{B}}
\newcommand{\bzero}{\boldsymbol{0}}

\newcommand{\bu} {\boldsymbol{u}}
\newcommand{\tbu} {\tilde{\boldsymbol{u}}}
\newcommand{\bt} {{\boldsymbol{t}}}
\newcommand{\btf} {{\boldsymbol{t}_f}}
\newcommand{\bbu} {\llbracket {\tbu}\rrbracket}
\newcommand{\bbut} {\llbracket {\bu}\rrbracket}
\newcommand{\brbu} {\llbracket {\breve\bu}\rrbracket}
\newcommand{\bv} {\boldsymbol{v}}
\newcommand{\Ga}{\G_{\mbox{\tiny{trial}}}}
\newcommand{\bxi} {\boldsymbol{\xi}}
\newcommand{\bxio} {\bxi\Zsup}
\newcommand{\tbv} {\tilde{\boldsymbol{v}}}
\newcommand{\Geps}{\Gamma_{\!\varepsilon}}
\newcommand{\bbb} {\llbracket\bar{\boldsymbol{v}}\rrbracket}
\newcommand{\bbv} {\llbracket {\tbv}\rrbracket}
\newcommand{\dbV} {\llbracket {V}\rrbracket}
\newcommand{\dbVe} {\llbracket {V_e}\rrbracket}
\newcommand{\dbVes} {\llbracket {V_{\nxs e^{\nxs*}}} \! \rrbracket}
\newcommand{\dbbV} {\llbracket {\boldsymbol{V}}\rrbracket}
\newcommand{\bR} {\boldsymbol{\sf R}}
% the definition of the cauchy principle value
\def\Xint#1{\mathchoice
{\XXint\displaystyle\textstyle{#1}}%
{\XXint\textstyle\scriptstyle{#1}}%
{\XXint\scriptstyle\scriptscriptstyle{#1}}%
{\XXint\scriptscriptstyle\scriptscriptstyle{#1}}%
\!\int}
\def\XXint#1#2#3{{\setbox0=\hbox{$#1{#2#3}{\int}$}
\vcenter{\hbox{$#2#3$}}\kern-.5\wd0}}
\def\ddashint{\Xint=}
\def\dashint{\Xint-}
\newcommand{\OOd}{\Omega}
\newcommand{\bpsi}{{\boldsymbol{\psi}}}
\setcounter{secnumdepth}{5}
\newcommand{\dualBR}[2]{\left< #1, #2 \right>_{\partial B_R}}
\newcommand{\hs}{\hspace{0.01 in}}  
\newcommand{\so}{{\text{\tiny o}}}  
\newcommand{\rstwo}{S_{_{\nxs \emph{\dva}}}}
\renewcommand{\topfraction}{1.0}
\renewcommand{\bottomfraction}{1.0}
\renewcommand{\textfraction}{0.0}
\newcommand{\bPhi}{\boldsymbol{\Phi}}
\newcommand{\lbreak}{\linebreak[4]}
\newcommand{\pbreak}{\pagebreak[4]}
%\newtheorem{theorem}{Theorem}[section]
%\newtheorem{lemma}[theorem]{Lemma}
%\newtheorem{prop}[theorem]{Proposition}
%\newtheorem{rem}{Remark}
%\newtheorem{corollary}{Corollary}
%\newtheorem{proof}{Proof}
\newcommand{\dualGA}[2]{\left< #1, #2 \right>_{\Gamma}}
%\newtheorem{rem}[ ]{Remark}
\newcommand{\bw} {\boldsymbol{w}}
\newenvironment{definition}[1][Definition]{\begin{trivlist}
\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
\newcommand{\btu} {\text{\bf{u}}}
\newcommand{\tSf}{\widetilde{\Sf}}
\newcommand{\ee}{{\text{\tiny \slshape{E}}}}
\newcommand{\TR}{{\mathcal T}_R}
 \newcommand{\bphi}{{\boldsymbol{\varphi}}}     
 \newcommand{\dbv} {\llbracket {\bv}\rrbracket}     
 \newcommand{\bfPsi}{\boldsymbol{\Psi}}
 \newcommand{\herg}{\mathcal{H}}
 \newcommand{\bh} {\boldsymbol{h}}
 
 
 
 
 
 
 
 
 
 
 
